Decidability, Complexity, and Expressiveness of First-Order Logic Over the Subword Ordering

We consider first-order logic over the subword ordering on finite words, where each word is available as a constant. Our first result is that the $\Sigma_1$ theory is undecidable (already over two letters). We investigate the decidability border by considering fragments where all but a certain number of variables are alternation bounded, meaning that the variable must always be quantified over languages with a bounded number of letter alternations. We prove that when at most two variables are not alternation bounded, the $\Sigma_1$ fragment is decidable, and that it becomes undecidable when three variables are not alternation bounded. Regarding higher quantifier alternation depths, we prove that the $\Sigma_2$ fragment is undecidable already for one variable without alternation bound and that when all variables are alternation bounded, the entire first-order theory is decidable.

==> app-complexity.tex <==
\subsection{Appendix on \cref{complexity}}

\subsubsection{Proof of \cref{thm:presburger-eq}}
\input{proof-interreduction-presburger.tex}


\iffalse
%
%
\subsubsection{Proof of \cref{complexity:subwords-in-presburger}
\input{proof-subwords-in-presburger.tex}
\fi %


\subsubsection{Proof of \cref{complexity:constraint-decomposition}}
\input{proof-constraint-decomposition.tex}

\subsubsection{Proof of \cref{complexity:two-variables:counterrelation}}

\input{lemma-counterautomata-emptiness.tex}

We are now ready to prove \cref{complexity:two-variables:counterrelation}.
\input{proof-twovariables-counterrelation.tex}




==> app-expressiveness.tex <==
\subsection{Appendix for \cref{expressiveness}}


\subsubsection{Proof of \cref{expressiveness:compatible}}\label{proof-expressiveness:compatible}
\input{proof-expressiveness-compatible.tex}


%
%

\subsubsection{Compatibility and recognizability}\label{app:compatibility:recognizability}
\input{theorem-compatibility-recognizability.tex}

%
%


\subsubsection{Proof of \cref{expressiveness:prefix}}
\input{proof-expressiveness-prefix.tex}



==> app-oneconstant.tex <==
\subsection{One constant is enough for undecidability}
%
\label{app-oneconstant}

We prove that the $\Sigma_1$ fragment can be undecidable with
$A=\{a,b\}$ even when only one constant $W\in A^*$ is available on the
condition that $W$ contains enough letters.

Recall that, in the proof of \Cref{subword:undecidable}, we use
constants to express PT properties like $x\in a^*$ or $u\in a^*b a a$ or
.. The most complex such properties are for points 4 and 5 of the
proof, where we use, e.g., $u\in a a b a^*b$, definable via
\[
a a b b\subword u
\land
b b b\not\subword u
\land
a a a b b\not\subword u
\land
b b a\not\subword u
\:.
\]
Therefore, undecidability for $\FO(A^*,\subword,W)$ will be provable
if we can define all words of length $\leq 5$ in the $\Sigma_1$
fragment, using only $W$.

So let us assume that $A=\{a,b\}$ and that $W$ is a word of length
$\ell$ with $|W|_a\geq 5$ and $|W|_b\geq 5$.  For any $i\leq \ell$, we
can define ``$x$ is a subword of length $i$ of $W$'' by
\[
\exists x_0,x_1,\ldots,x_\ell:
x_0 \strictsubword
x_1\strictsubword x_2 \strictsubword \cdots
\strictsubword x_\ell=W
\land x=x_i\:.
\]
In particular, we can define $\epsilon$ and the two letters $a$ and
$b$ up to a bijective renaming of letters that we now assume w.l.o.g.\ is
the identity.


Since $|W|_a\geq 5$ we can define $a a$ as a subword of $W$ of length 2
that does not contain $b$.  Similarly we can define any $a^i$ or $b^i$
for $i=2,\ldots,5$.

We can define $a b$ and $b a$ as the only two distinct words that have
one $a$ and one $b$ (they don't have to be subwords of $W$).  This is
up to an automorphism that can be the reversal operation or the
identity. As above, we shall assume that this automorphism is the identity.


We can further define
$x=a a b$ e.g. with
\[
a a\subword x\land a a a\not\subword x
\land a b\subword x\land b b\not\subword x
\land b a\not\subword x\:,
\]
and similarly for $a b a$, $b b a$, etc.

We can then define all words of $A^{=i}$ for $i=4$ and $5$ by
specifying their lengths (specifying the number of $a$'s and the
number of $b$'s) and their subwords of length $i-1$.

When $W=\epsilon$, the decidability proof (from~\cite{kuske2006}) for
$\Sigma_1$ formulas without constants is easy to extend.


%
%
%
%
%




==> proof-interreduction-presburger.tex <==
\begin{proof}
Let $\theta$ be a closed $\frag{i}{0}$ formula. Let $\ell$ be the maximum
alternation of all variables quantified in $\theta$. Consider the formula
$\theta'$ obtained from $\theta$ by replacing every quantification $Q x \in
(a_1^* \cdots a_n^*)^{\ell_x}$ by $Q x_{1,1}, \dots, x_{\ell,n} \colon
\bigwedge_{\substack{\ell_x < i \le \ell}{1 \le j \le n}} x_{i,j} = 0$ and
literals $x \subword y$ and $x \not\subword y$ by $\varphi(x_{1,1}, \dots,
x_{\ell,n}, y_{1,1}, \dots, y_{\ell,n})$ and $\psi(x_{1,1}, \dots, x_{\ell,n},
y_{1,1}, \dots, y_{\ell,n})$, respectively. Then by
\cref{subwords-in-presburger}, the validity of $\theta$ and $\theta'$ are
equivalent.


On the other hand, the proof of \cref{subword:undecidable} shows that we can
express addition in $\frag{1}{0}$ if $|A|\ge 2$. Since ``$|u|_a \ne |v|_a$'' is
expressible in $\Sigma_1$, we can also express ``$|w|_a\ne |u|_a+|v|_a$'' in
$\Sigma_1$.  Thus, we can
express addition in $\Pi_1$.  Together, this means the $\Sigma_i$ fragment of
Presburger arithmetic can be reduced in polynomial time to the $\frag i 0$
fragment of subwords.  The complexity of the $\Sigma_i$ fragment of Presburger
arithmetic is settled in \cite{Haase2014}.
\end{proof}




==> proof-subwords-in-presburger.tex <==
\begin{proof}
%
%
%
%

Since the formula $\psi$ is equivalent to the negation of $\varphi$, it
suffices to show the correctness of $\varphi$.

Subsequently, we will denote factors of $w_x$ (\emph{resp.} $w_y$) of the form $a_j^{x_{i,j}}$ (\emph{resp.} $a_j^{y_{i,j}}$) as factor $x_{i,j}$ (\emph{resp.} $y_{i,j}$).

Assume $w_x \subword w_y$. Let $f$ be the left-most embedding of $w_x$ into $w_y$.
%
Let $w_x^i$ (\emph{resp.} $w_y^i$) denote $a_1^{x_{1,1}} \cdots a_n^{x_{i-1,n}}$ (\emph{resp.} $y_{1,1} \cdots y_{i-1,n}$), \emph{i.e.} the prefix of $w_x$ which consists of the $(i-1)-th$ first alternations.
Let $e_{i,j,k}$ be the number of letters from factor $x_{i,j}$ of $w_x$ that are mapped vy $f$ to some letter from factor $y_{k,j}$ of $w_y$. Define:
\begin{align*}
  t_{i,j,k} = \begin{cases}
    0 &\text{ if } w_x^i \not\subword w_y^{k+1} \\
    y_{k,j} - \sum_{i' =1}^{i-1} e_{i',j,k} &\text{ otherwise }
  \end{cases}
\end{align*}

Formula $\xi$ is then satisfied: let $(i,j,k) \in I\times [1,\ell]$. Assume that there exists $(i',j') < (i,j)$ and $k' > k$ such that $e_{i',j',k'} > 0$. By definition, this means that the embedding $f$ maps some letters of $x_{i',j'}$ to some letters of $y_{k',j'}$. Since $f$ is left-most and $k' > k$, this implies that $w_x^i \not\subword w_y^{k+1}$. Thus, $t_{i,j,k}$ is indeed equal to $0$. Otherwise, this means that no symbol on the left of $x_{i,j}$ is mapped by $f$ to a symbol on the right of $y_{k,j}$, hence ${w_x}^i \subword w_y^{k+1}$. Thus, our definition of $t_{i,j,k}$ satisfy formulas $\tau_{i,j}$ for every $(i,j)\in I$.

For the second conjunction of $\xi$, let $(i,j,k) \in I \times [1,\ell]$. Depending on the value of $t_{i,j,k}$:
\begin{enumerate}
\item If ${w_x}^i \not\subword {w_y}^{k+1}$, \emph{i.e.} $t_{i,j,k} = 0$, then as seen above, elements of $x_{i,j}$ cannot be mapped to $y_{k,j}$, hence $e_{i,j,k} = 0$.
\item Otherwise, if $x_{i,j} - \sum_{r=1}^{k-1} e_{i,j,r} \le t_{i,j,k} = y_{k,j} - \sum_{i'=1}^i e_{i',j,k}$ then it means that the number of letters in $y_{k,j}$ that are not in the image of ${w_x}^i$ by function $f$ is greater than the number of letters of factor $x_{i,j}$ that are not mapped by $f$ to a factor on the left of $y_{k,j}$. Thus, since $f$ is left-most, all these letters from $x_{i,j}$ are mapped into $y_{k,j}$, and $e_{i,j,k} = x_{i,j} - \sum_{r=1}^{k-1} e_{i,j,r}$. The case where $x_{i,j} - \sum_{r=1}^{k-1} e_{i,j,r} \ge t_{i,j,k} = y_{k,j} - \sum_{i'=1}^i e_{i',j,k}$ is similar.
\end{enumerate}

Finally, our definition of $e_{i,j,k}$ and the fact that $w_x \subword w_y$ entails that for every $i,j$, $x_{i,j} \le \sum_{k=1}^\ell e_{i,j,k}$ (this even is an equality).

Conversely, if $\varphi$ is satisfied, we show that the function $f$ that maps $e_{i,j,k}$ letters from factor $x_{i,j}$ to $y_{k,j}$ is a valid embedding of $w_x$ into $w_y$. Since for every $(i,j) \in I$, $x_{i,j} \le \sum_{k=1}^l e_{i,j,k}$, every letter of $w_x$ is mapped to some letter of $w_y$. Moreover, there are enough letters in $w_y$ for $f$ to be injective, that is for every $(k,j) \in I$, $\sum_{i=1}^l e_{i,j,k} \le y_{k,j}$. The latter hold since by formula $\xi$, $e_{\ell,j,k} \le t_{\ell,j,k} \le y_{k,j} - \sum_{i = 1}^{\ell - 1} e_{i,j,k}$, from which we derive the desired inequality. Finally, it remains to show that the embedding is increasing, that is for every $(i,j,k)$, $e_{i,j,k} \neq 0$ implies that for every $(i',j') < (i,j)$ and $k' > k$, $e_{i',j',k'} = 0$. This implication holds since whenever there exists $(i',j') < (i,j)$ and $k' < k$ such that $e_{i',j',k'} \neq 0$, $t_{i,j,k} = 0$ by formula $\tau_{i,j}$ and thus $e_{i,j,k} = 0$ by formula $\eta_{i,j}$.
\end{proof}




==> sec-acknow.tex <==
\section*{Acknowledgments}
%
The authors would like to thank...



